A simple way to compute structure constants of semi-simple Lie algebras

The standard way to compute the structure constants of semi-simple Lie algebras involves the additive structure of the roots. In earlier work, I described how ideas of Jacques Tits could be applied to do this by using the structure of the Weyl group. In this work, I explain how to combine some of the earlier ideas with some suggestions of Kottwitz to present a very simple algorithm which comes close to constructing a canonical basis of the Lie algebra. Unfortunately, unlike previous methods, it does not work for arbitrary Kac-Moody algebra.

==> k.tex <==




==> labels/klbls.tex <==
\expandafter \def \csname satz-KottwitzConstants-change\endcsname {Lemma 1.1}
\expandafter \def \csname localsatz-KottwitzConstants-change\endcsname {Lemma 1.1}
\expandafter \def \csname satz-KottwitzConstants-integral-basis\endcsname {Definition 1.2}
\expandafter \def \csname localsatz-KottwitzConstants-integral-basis\endcsname {Definition 1.2}
\expandafter \def \csname satz-KottwitzConstants-cheveq\endcsname {(1.3) }
\expandafter \def \csname localsatz-KottwitzConstants-cheveq\endcsname {(1.3)}
\expandafter \def \csname satz-KottwitzConstants-plambdamu\endcsname {(1.4) }
\expandafter \def \csname localsatz-KottwitzConstants-plambdamu\endcsname {(1.4)}
\expandafter \def \csname satz-KottwitzConstants-tits-cts\endcsname {Lemma 2.1}
\expandafter \def \csname localsatz-KottwitzConstants-tits-cts\endcsname {Lemma 2.1}
\expandafter \def \csname satz-KottwitzConstants-fef\endcsname {(2.2) }
\expandafter \def \csname localsatz-KottwitzConstants-fef\endcsname {(2.2)}
\expandafter \def \csname satz-KottwitzConstants-compatibility\endcsname {Lemma 2.3}
\expandafter \def \csname localsatz-KottwitzConstants-compatibility\endcsname {Lemma 2.3}
\expandafter \def \csname satz-KottwitzConstants-practical\endcsname {Lemma 2.4}
\expandafter \def \csname localsatz-KottwitzConstants-practical\endcsname {Lemma 2.4}
\expandafter \def \csname satz-KottwitzConstants-tits-tfae\endcsname {Proposition 2.5}
\expandafter \def \csname localsatz-KottwitzConstants-tits-tfae\endcsname {Proposition 2.5}
\expandafter \def \csname satz-KottwitzConstants-tits-f\endcsname {Proposition 2.6}
\expandafter \def \csname localsatz-KottwitzConstants-tits-f\endcsname {Proposition 2.6}
\expandafter \def \csname satz-KottwitzConstants-rotation\endcsname {Proposition 2.7}
\expandafter \def \csname localsatz-KottwitzConstants-rotation\endcsname {Proposition 2.7}
\expandafter \def \csname satz-KottwitzConstants-abc-cor\endcsname {Theorem 2.8}
\expandafter \def \csname localsatz-KottwitzConstants-abc-cor\endcsname {Theorem 2.8}
\expandafter \def \csname satz-KottwitzConstants-summary1\endcsname {Theorem 3.1}
\expandafter \def \csname localsatz-KottwitzConstants-summary1\endcsname {Theorem 3.1}
\expandafter \def \csname satz-KottwitzConstants-rsw\endcsname {(4.1) }
\expandafter \def \csname localsatz-KottwitzConstants-rsw\endcsname {(4.1)}
\expandafter \def \csname satz-KottwitzConstants-ca\endcsname {(4.2) }
\expandafter \def \csname localsatz-KottwitzConstants-ca\endcsname {(4.2)}
\expandafter \def \csname satz-KottwitzConstants-cb\endcsname {(4.3) }
\expandafter \def \csname localsatz-KottwitzConstants-cb\endcsname {(4.3)}
\expandafter \def \csname satz-KottwitzConstants-w-invariance\endcsname {Lemma 4.4}
\expandafter \def \csname localsatz-KottwitzConstants-w-invariance\endcsname {Lemma 4.4}
\expandafter \def \csname satz-KottwitzConstants-cc\endcsname {(4.5) }
\expandafter \def \csname localsatz-KottwitzConstants-cc\endcsname {(4.5)}
\expandafter \def \csname satz-KottwitzConstants-kottwitz\endcsname {Theorem 4.6}
\expandafter \def \csname localsatz-KottwitzConstants-kottwitz\endcsname {Theorem 4.6}
\expandafter \def \csname satz-KottwitzConstants-kottwitz-basis\endcsname {Corollary 4.7}
\expandafter \def \csname localsatz-KottwitzConstants-kottwitz-basis\endcsname {Corollary 4.7}
\expandafter \def \csname satz-KottwitzConstants-semi-can\endcsname {Definition 4.8}
\expandafter \def \csname localsatz-KottwitzConstants-semi-can\endcsname {Definition 4.8}
\expandafter \def \csname satz-KottwitzConstants-sl3-e\endcsname {Proposition 4.9}
\expandafter \def \csname localsatz-KottwitzConstants-sl3-e\endcsname {Proposition 4.9}
\expandafter \def \csname satz-KottwitzConstants-ht-parity\endcsname {Theorem 4.10}
\expandafter \def \csname localsatz-KottwitzConstants-ht-parity\endcsname {Theorem 4.10}
\expandafter \def \csname satz-KottwitzConstants-theta-Ddot\endcsname {(4.11) }
\expandafter \def \csname localsatz-KottwitzConstants-theta-Ddot\endcsname {(4.11)}
\expandafter \def \csname satz-KottwitzConstants-ea-lemma\endcsname {Corollary 4.12}
\expandafter \def \csname localsatz-KottwitzConstants-ea-lemma\endcsname {Corollary 4.12}
\expandafter \def \csname satz-KottwitzConstants-T-basis\endcsname {Proposition 5.1}
\expandafter \def \csname localsatz-KottwitzConstants-T-basis\endcsname {Proposition 5.1}
\expandafter \def \csname satz-KottwitzConstants-basic-formula\endcsname {Theorem 5.2}
\expandafter \def \csname localsatz-KottwitzConstants-basic-formula\endcsname {Theorem 5.2}


==> labels/ktoc.tex <==
\advance \SEC by 1
\hskip 2em\ifnum \SEC < 10 \kern 1ex\else \kern 0ex\fi 
\the \SEC 
. Chevalley bases\leaders \hbox to 1ex{\hss .\hss }\hfill \kern 1ex 3\hskip 3em\hbox {}\kern 1ex\par 
\advance \SEC by 1
\hskip 2em\ifnum \SEC < 10 \kern 1ex\else \kern 0ex\fi 
\the \SEC 
. Tits' idea\leaders \hbox to 1ex{\hss .\hss }\hfill \kern 1ex 5\hskip 3em\hbox {}\kern 1ex\par 
\advance \SEC by 1
\hskip 2em\ifnum \SEC < 10 \kern 1ex\else \kern 0ex\fi 
\the \SEC 
. Computation I\leaders \hbox to 1ex{\hss .\hss }\hfill \kern 1ex 8\hskip 3em\hbox {}\kern 1ex\par 
\advance \SEC by 1
\hskip 2em\ifnum \SEC < 10 \kern 1ex\else \kern 0ex\fi 
\the \SEC 
. Kottwitz' splittings\leaders \hbox to 1ex{\hss .\hss }\hfill \kern 0ex 10\hskip 3em\hbox {}\kern 1ex\par 
\advance \SEC by 1
\hskip 2em\ifnum \SEC < 10 \kern 1ex\else \kern 0ex\fi 
\the \SEC 
. Computation II\leaders \hbox to 1ex{\hss .\hss }\hfill \kern 0ex 16\hskip 3em\hbox {}\kern 1ex\par 
\advance \SEC by 1
\hskip 2em\ifnum \SEC < 10 \kern 1ex\else \kern 0ex\fi 
\the \SEC 
. Summary\leaders \hbox to 1ex{\hss .\hss }\hfill \kern 0ex 18\hskip 3em\hbox {}\kern 1ex\par 
\advance \SEC by 1
\hskip 2em\ifnum \SEC < 10 \kern 1ex\else \kern 0ex\fi 
\the \SEC 
. References\leaders \hbox to 1ex{\hss .\hss }\hfill \kern 0ex 18\hskip 3em\hbox {}\kern 1ex\par 


==> macros/colordvi.tex <==
% This is COLORDVI.TEX and COLORDVI.STY in text format, as of
% March 5, 1992, written by Jim Hafner, HAFNER@ALMADEN, or
% hafner@almaden.ibm.com.  Modified by Tomas Rokicki to be a
% bit smaller and easier to add to.
%
% 20 Aug. 1992: Revised by J. Hafner, by adding \globalColor.
%
% This style file can be used to get color in TeX, LaTeX or more
% importantly, FoilTeX as an optional style file.  It is generic in
% that the color parameters are determined by the driver's header files.
%
% It can be used with any driver which knows how to process the keywords
% in the \special commands.  Currently, only versions of dvips greater
% than 5.478 (dvips is the DVI->PostScript driver by Tom Rokicki) and
% TeXview on the NeXT interpret these specials.
%
% This file can be used in any flavor of LaTeX (e.g. LaTeX, FoilTeX,
% AMS-LaTeX) by adding the keyword "colordvi" to the options in the
% \documentstyle command (e.g., "\documentstyle[colordvi]{foils}") or \input
% in any flavor of TeX (e.g. Plain TeX, eplain, AMS-TeX or any of the
% above LaTeX flavors) with the command "\input colordvi".
%
% The actual parameters for each color are determined by the device
% driver.
% For "dvips", that is the header file color.pro prepended to the
% output file by dvips.  They can be overrriden by a user-supplied
% header, called by either the -h option or the "h" flag in a printer
% configuration file, or in the .dvipsrc (or its analogue on other
% systems).
%
% Most of the color names and their matches were based on the
% most recent (at time of writing) Crayola Crayon box of 64 colors.
%
% There are 68 predefined colors.  At the end of this file is a
% listing of the color names and their approximate PANTONE color
% match.  This is for reference purposes only.
%
% The first macro lets the user specify the background color for the
% document.  It sets the background color for the current page and all
% succeeding pages, unless changed by another command of this type.  To
% change the background color back to the default, issue
% \background{White}
%
\def\background#1{\special{background #1}}
%
% There are two types of text color commands.  The first is in the form
%    \ColorName   (note the uppercase for the color name).
%
% It is called a local color command since it takes one argument
% enclosed in brackets.  It writes the contents of its argument in the
% selected color.  This should be used for local or nested color
% changes, since it restores the original color state when it completes.
% The second type of color command is in the form
%    \textColorName
% This uses the same naming convention as before.  It is called a global
% color command since it takes no arguments and simply sets the color at
% this point.  No previous color information is saved.  IF YOU USE THIS
% INTERNAL TO ANY LOCAL COLOR COMMAND, THE NESTING HISTORY IS LOST.
%
% This next definition is used in an invocation of a \textColorName
% macro to save the global color value in local form via the \globalColor
% macro.  This new macro can then be used to protect certain regions of
% the text, like item tags and headers and footers which can be
% corrupted by local colors.  In particular, item tags in lists can
% incorrectly inherit the color from a local color command immediately
% following it.  The \subdef macro is invoked within the invocation of a
% global color change.
%
\def\subdef#1{\gdef\globalColor##1{\special
       {color push #1}##1\special{color pop}}}
%
% Here are the global color changers, with color codes defined;
% these are used to define the small region colors.
%
% This first is for user defined color.  The argument #1 is for a "CMYK"
% quadruple of intensity values between 0 and 1.  (CMYK stands for Cyan,
% Magenta, Yellow and Black.)  E.g., \textColor{.2 .3 .4 .1}
%
\def\textColor#1{\subdef{cmyk #1}\special{color cmyk #1}}
%
% and a userdefinable local color command.
\def\Color#1#2{\special{color push cmyk #1}#2\special{color pop}}
%
%
\def\newColor #1 {\expandafter\def\csname #1\endcsname##1{\special
   {color push #1}##1\special{color pop}}%
   \expandafter\def\csname text#1\endcsname{\subdef{#1}%
    \special{color #1}}}%
%
% Here are the color names and their PANTONE match (approximately)
%
\newColor GreenYellow     % GreenYellow  Approximate PANTONE 388
\newColor Yellow	  % Yellow  Approximate PANTONE YELLOW
\newColor Goldenrod	  % Goldenrod  Approximate PANTONE 109
\newColor Dandelion	  % Dandelion  Approximate PANTONE 123
\newColor Apricot	  % Apricot  Approximate PANTONE 1565
\newColor Peach		  % Peach  Approximate PANTONE 164
\newColor Melon		  % Melon  Approximate PANTONE 177
\newColor YellowOrange	  % YellowOrange  Approximate PANTONE 130
\newColor Orange	  % Orange  Approximate PANTONE ORANGE-021
\newColor BurntOrange	  % BurntOrange  Approximate PANTONE 388
\newColor Bittersweet	  % Bittersweet  Approximate PANTONE 167
\newColor RedOrange	  % RedOrange  Approximate PANTONE 179
\newColor Mahogany	  % Mahogany  Approximate PANTONE 484
\newColor Maroon	  % Maroon  Approximate PANTONE 201
\newColor BrickRed	  % BrickRed  Approximate PANTONE 1805
\newColor Red		  % Red  VERY-Approx PANTONE RED
\newColor OrangeRed	  % OrangeRed  No PANTONE match
\newColor RubineRed	  % RubineRed  Approximate PANTONE RUBINE-RED
\newColor WildStrawberry  % WildStrawberry  Approximate PANTONE 206
\newColor Salmon	  % Salmon  Approximate PANTONE 183
\newColor CarnationPink	  % CarnationPink  Approximate PANTONE 218
\newColor Magenta	  % Magenta  Approximate PANTONE PROCESS-MAGENTA
\newColor VioletRed	  % VioletRed  Approximate PANTONE 219
\newColor Rhodamine	  % Rhodamine  Approximate PANTONE RHODAMINE-RED
\newColor Mulberry	  % Mulberry  Approximate PANTONE 241
\newColor RedViolet	  % RedViolet  Approximate PANTONE 234
\newColor Fuchsia	  % Fuchsia  Approximate PANTONE 248
\newColor Lavender	  % Lavender  Approximate PANTONE 223
\newColor Thistle	  % Thistle  Approximate PANTONE 245
\newColor Orchid	  % Orchid  Approximate PANTONE 252
\newColor DarkOrchid	  % DarkOrchid  No PANTONE match
\newColor Purple	  % Purple  Approximate PANTONE PURPLE
\newColor Plum		  % Plum  VERY-Approx PANTONE 518
\newColor Violet	  % Violet  Approximate PANTONE VIOLET
\newColor RoyalPurple	  % RoyalPurple  Approximate PANTONE 267
\newColor BlueViolet	  % BlueViolet  Approximate PANTONE 2755
\newColor Periwinkle	  % Periwinkle  Approximate PANTONE 2715
\newColor CadetBlue	  % CadetBlue  Approximate PANTONE (534+535)/2
\newColor CornflowerBlue  % CornflowerBlue  Approximate PANTONE 292
\newColor MidnightBlue	  % MidnightBlue  Approximate PANTONE 302
\newColor NavyBlue	  % NavyBlue  Approximate PANTONE 293
\newColor RoyalBlue	  % RoyalBlue  No PANTONE match
\newColor Blue		  % Blue  Approximate PANTONE BLUE-072
\newColor Cerulean	  % Cerulean  Approximate PANTONE 3005
\newColor Cyan		  % Cyan  Approximate PANTONE PROCESS-CYAN
\newColor ProcessBlue	  % ProcessBlue  Approximate PANTONE PROCESS-BLUE
\newColor SkyBlue	  % SkyBlue  Approximate PANTONE 2985
\newColor Turquoise	  % Turquoise  Approximate PANTONE (312+313)/2
\newColor TealBlue	  % TealBlue  Approximate PANTONE 3145
\newColor Aquamarine	  % Aquamarine  Approximate PANTONE 3135
\newColor BlueGreen	  % BlueGreen  Approximate PANTONE 320
\newColor Emerald	  % Emerald  No PANTONE match
\newColor JungleGreen	  % JungleGreen  Approximate PANTONE 328
\newColor SeaGreen	  % SeaGreen  Approximate PANTONE 3268
\newColor Green		  % Green  VERY-Approx PANTONE GREEN
\newColor ForestGreen	  % ForestGreen  Approximate PANTONE 349
\newColor PineGreen	  % PineGreen  Approximate PANTONE 323
\newColor LimeGreen	  % LimeGreen  No PANTONE match
\newColor YellowGreen	  % YellowGreen  Approximate PANTONE 375
\newColor SpringGreen	  % SpringGreen  Approximate PANTONE 381
\newColor OliveGreen	  % OliveGreen  Approximate PANTONE 582
\newColor RawSienna	  % RawSienna  Approximate PANTONE 154
\newColor Sepia		  % Sepia  Approximate PANTONE 161
\newColor Brown		  % Brown  Approximate PANTONE 1615
\newColor Tan		  % Tan  No PANTONE match
\newColor Gray		  % Gray  Approximate PANTONE COOL-GRAY-8
\newColor Black		  % Black  Approximate PANTONE PROCESS-BLACK
\newColor White		  % White  No PANTONE match

% Now we make sure that we initialize the global color to Black
\subdef{Black}


==> macros/layout.tex <==

% --- look of the pages -------------------------------

\def\Romannumeral#1{\uppercase\expandafter{\romannumeral #1}}

\def\makeheadline{\vbox to 0pt{\vss\noindent
% later pages:
\ifnum\pageno>1
\Black{{\leavevmode\kern-\parindent\rm\runningtitle \ \ \ifproofmode(\now\ \ \today)\else\null\fi}}\hfill{\rm \Black{\folio}}
\else% first page:
\Black{%\write16{\the\parindent} 
% \ifproofmode\kern-\parindent{\tt \filename.tex}
\ifproofmode{\tt \filename.tex}
\kern\parindent\else\null\fi\hfill\rm Last revised \now\ \ \today}\hfill\fi}%
%
\ifnum\pageno<2 \vskip3pt\Black{\hrule}\vskip\baselineskip
% \ifnum\pageno<2 \vskip3pt\Black{\hrule}\vskip\baselineskip
\else\vskip3pt\Black{\hrule}\vskip\baselineskip%
\fi%
}% 

\def\makefootline{}

\newcount\SEC

\def\contents {

{\bold Contents}

\medskip

\begingroup
\parskip=0pt
\input \tocfile
\endgroup

\immediate\openout\toc=\tocfile.tex
\immediate\write\toc{\SEC=0}%
}

% ---------------------------------------------

\newif
\ifsectionbreak
\sectionbreakfalse

\newif
\ifinparttitle
\inparttitlefalse

\newif
\ifjustafter
\justafterfalse

\newcount\partno
\partno=0

\def\part#1{
\global\advance\partno by 1
% \immediate
\write\toc{\hskip0em\uppercase\expandafter{\romannumeral\partno}. #1\par}
% \ifproofmode\ifodd\pageno\vfill\eject\null\vfill\eject\else\vfill\eject\fi\else\vskip0.25truein\fi
\ifsectionbreak \vfill\break \else \goodbreak \fi
% \goodbreak
\bigskip
\centerline{{\bold Part \uppercase\expandafter{\romannumeral\partno}. #1\ }}
\justaftertrue
}

\newif
\ifinchaptertitle
\inchaptertitlefalse
\newif
\ifinsectiontitle
\insectiontitlefalse

\newif\ifinchapter
\newif\ifinapp
\newif\ifinsec
\newif\ifinsubsec

\newcount\chapterno
\chapterno=0

\newcount\satzno
\satzno=0

\newcount\secno
\secno=0

\newcount\appno
\appno=0

\newcount\subsecno
\subsecno=0

\newcount\exno
\exno=0

\def\exer#1{\advance\exno by 1 {\bold Exercise \the\secno.\the\exno. \sl #1}} 

% - chapters ----------------------------------------

\newcount\chapterno
\chapterno=0

\def\chapter#1#2{
\chapterno=#1
\inchaptertrue
\satzno=0
\exno=0
\secno=0
\bigbreak{\bigbold Chapter \Romannumeral{#1}. #2}\inchaptertitlefalse
\gdef\runningtitle{Chapter \Romannumeral{#1}. #2}
\nobreak\medbreak\nobreak}

\def\endchapter{\vfill\eject}

% - sections ------------------------------------

\def\iw{\write}

% #1 = \the secno, #2 = title
\def\writeS#1#2{%
%
% \write16{*** #1 ***}
\iw\toc{\advance\SEC by 1}
\iw\toc{\hskip2em%
%\ifinchapter\Romannumeral{\the\chapterno}.\fi%
% \ifnum\secno < 10 \kern1ex\else\kern0ex\fi\the\secno. #1\leaderfill 
\noexpand\ifnum\noexpand\SEC < 10 \noexpand\kern1ex\noexpand\else\noexpand\kern0ex\noexpand\fi}%
\iw\toc{\noexpand\the\noexpand\SEC}%
\iw\toc{. #2\leaderfill 
\ifnum\pageno<10 \kern1ex \else\kern0ex \fi \the\pageno\hskip3em\null\kern1ex\par}%
%
}

\def\subfilename{\filename}

\def\intro{\immediate\write\tocout{ \ifnum\secno < 10 --- \else -- \fi Introduction --- }
\immediate\write\toc{Introduction\par}
\ifproofmode\vfill\eject\else\bigbreak\fi
{\bold Introduction}
\nobreak\medbreak\nobreak}

\def\leaderfill{\leaders\hbox to 1ex{\hss.\hss}\hfill }

\def\section#1{
\ifjustafter \justafterfalse \else \ifsectionbreak \vfill\eject \else \goodbreak \fi \fi
\global\advance\secno by 1

% \immediate\write16{........... [Section \the\secno ] #1 ........... }

\exno=0
\satzno=0
\subsecno=0 %\immediate
\write\tocout{ \ifnum\secno < 10 --- \else --- \fi\the\secno. #1 --- }
%
\insectiontitletrue
\medbreak{\bold \the\secno. #1 \ifproofmode{\tt [\subfilename.tex]}\else\fi}
\insectiontitlefalse
\inappfalse
\insubsecfalse
\insectrue
\nobreak\medbreak\nobreak
%
% old problem: 
% \immediate\write doesn't get pageno right
% \write doesn't get \secno right
% fixed by writing macros into toc file
%
\writeS{\expandafter\the\secno}{#1}
}

\def\appendix#1{%
\section{{\sl Appendix.} #1}}

% ---------------------------------------------------

\def\subsection#1{
\satzno=0
\advance\subsecno by 1
\goodbreak
 % \medbreak{\bold \ifinapp A.\fi\ifinsec\the\secno.\fi\the\subsecno. #1}
\smallbreak{\bold #1}
\insubsectrue}
\def\endsubsection{\insubsecfalse}
\def\endsection{\insecfalse}


\def\introduction{
\satzno=0
\goodbreak
\inappfalse
\insubsecfalse
\insecfalse
\medbreak{\bold Introduction}
\nobreak\medbreak\nobreak}

\input macros/satzen

% ------------------------------------------------------------------

\def\subsec#1{\BrickRed{{\bigsc \uppercase{#1}}.\ }}
\def\subtitle#1{{\sl #1}.\ }

\def\qed{\hbox{\frenchspacing\sc\ Q.E.D.}}
\def\proof/{{\sl Proof}}

\def\emptybox#1#2{\relax
\dimen1=#1pt\advance\dimen1 by #2pt%
\advance\dimen1 by #2pt%
\hbox{%
\hskip 1pt
\vbox{\hrule width \dimen1 height #2pt%
\hbox{\vrule height #1pt width #2pt \kern #1pt%
\vrule height #1pt width #2pt}%
\hrule width \dimen1 height #2pt}}}

\def\endproof{\null\hfill~\raise-1pt\hbox{\epsfbox{macros/redbox.eps}}\null}
\def\mendproof{\eqno\hfill\raise-1pt\hbox{\epsfbox{macros/redbox.eps}}}
\def\dblendproof{\null\hfill~\raise-1pt\hbox{\epsfbox{macros/redbox.eps}\epsfbox{macros/redbox.eps}}\null}
\def\dblmendproof{\eqno\hfill~\raise-1pt\hbox{\epsfbox{macros/redbox.eps}\epsfbox{macros/redbox.eps}}}

% --------------------------------------------

\def\today{\ifcase\month\or January\or February\or March\or
April\or May\or June\or July\or August\or September\or
October\or November\or December\fi
\space\number\day, \number\year}

\def\now{\begingroup
\count0 = \time
\divide\count0 by 60 % the hour
\count2 = \count0
\count4 = \time
\multiply\count0 by 60
\advance\count4 by -\count0 % the minute
\ifnum\count4<10 \toks1={0}%
\else			 \toks1={}%
\fi
\ifnum\count2<12 \toks0 = {a.m.}%
\else			 \toks0={p.m.}%
\advance\count2 by -12
\fi
\ifnum\count2=0 \count2=12 \fi % midnight = 12
\number\count2:\the\toks1 \number\count4\thinspace\the\toks0
\endgroup}
%

\def\dendproof#1{\null
\vskip-#1\baselineskip
\null\hfill\endproof\null
\par}

\def\strutdepth{\dp\strutbox}
\def\margininsert#1{\strut\vadjust{\kern-\strutdepth
\vtop to \strutdepth{%
\baselineskip\strutdepth\vss\llap{\smallfont #1}\null}}}
%
\def\margininserts#1#2{\strut\vadjust{\kern-1\strutdepth\kern-\baselineskip
\vtop to \strutdepth{\baselineskip\strutdepth\vss\llap{\smallfont #1}\null}
\vtop to \strutdepth{\baselineskip\strutdepth\vss\llap{\smallfont #2}\null}}}

\def\scr{\scriptstyle}
\def\sscr{\scriptscriptstyle}

\def\note#1{\ifproofmode%
$\null^{\circ}$\kern-4pt
\setbox0\vbox{\overfullrule=0pt
\hsize=1truein
\parindent=0pt
\baselineskip=9pt
\raggedright
$\scr\langle\k{-2}\langle$\smallrmfont #1$\scr\rangle\k{-2}\rangle$}
\margininsert{\BrickRed{\box0}\ }%
\fi}

\def\query{\ifproofmode%
$\null^{\circ}$\kern-4pt
\setbox0\vbox{\overfullrule=0pt
\hsize=1truein
\parindent=0pt
\baselineskip=9pt
\raggedright
$\diamondsuit\diamondsuit\diamondsuit$}
\margininsert{\BrickRed{\box0}\ }%
\fi}

% --- references ---------------------------------------------------
% The macros in this file handle references by filename, both bibliography and theorems.
% This file also opens the files "satzlbls.tex" and "reflbls.tex" where the definitions are stored.
% --- internal -----------------------------------------------------

\def\ifempty#1{\xifempty #1\xemptymarkA\xemptymarkB}%

\def\xifempty#1#2\xemptymarkB{\ifx #1\xemptymarkA}%

\def\xemptymarkA{\xemptymarkA}%

\def\tokstostring#1{\ttsA#1 \endttsA}%

\def\ttsA#1 #2\endttsA{\ifempty{#1}\else
\ttsB #1\endttsB
\ifempty{#2}\else
\spacesub\ttsA#2\endttsA\fi\fi}%

\def\ttsB#1{\ifx #1\endttsB\else
\string #1%
\expandafter\ttsB\fi}%

\def\endttsB{\endttsB}%

% ------------------------------------------------

\def\references{\input macros/ref.macros
\ifnum\secno > 0 \section{References} \else {\goodbreak\bold References\bigskip} \fi}

\def\referencespart{\input macros/ref.macros
\part{References}}

\def\loadrefmacs{\input macros/ref.macros}

\def\localreferences{\BrickRed{{\bigsc REFERENCES}}}

\def\References{\input macros/ref.macros
\ifsectionbreak \vfill\eject \fi
\part{References}}

% ------------------------------------------------

\def\itema{\item{(\kern0.6pt a\kern0.6pt )}}
\def\itemb{\item{(\kern1.0pt b)}} 
\def\itemc{\item{(\kern1.0pt c\kern0.8pt )}} 
\def\itemd{\item{(\kern0.3pt d\kern0.3pt)}} 
\def\iteme{\item{(e)}} 
\def\itemf{\item{(f)}}

% ------------------------------------------------

\def\figure#1{\leavevmode
\null
\hfill
\epsfbox{#1}\ifproofmode\margininsert{{\marginbf #1}}\fi
\hfill
\null}

\def\figures#1#2{\leavevmode
\hfill
\epsfbox{#1}
\hfill
\epsfbox{#2}
\hfill
\null
\setbox0=\vbox{#1\hfill\break XXX #2}
\ifproofmode\margininserts{{\marginbf #1}}{{\marginbf #2}}\fi}

\def\Ie/{{\frenchspacing I. e.}}

\newcount\stepno
\stepno = 0
\def\step{\advance\stepno by 1{\bold Step \the\stepno.} }

\def\mmatrix#1{\left[\matrix { #1 } \right]}
\def\Cdot{\kern-1pt \cdot \kern-1pt}
\def\newpage{\vfill\eject}

\def\author{
Bill Casselman\hfill\break
University of British Columbia\hfill\break
{\tt cass@math.ubc.ca}
}

\def\hbreak{\bigskip\hrule\bigskip}
\def\refto#1#2{[#1:#2]}
\def\frechet/{Fr\'echet}
\def\milicic/{Mili\v ci\'c}

\def\beginitems#1{\begingroup
\parskip=0pt
\parindent=#1}
\def\enditems{\endgroup}

\def\TILDE{\raise-3pt\hbox{\tt \char126}}
\def\AT{\raise-3pt\hbox{\tt\char126}\kern0.5pt}

\def\k#1{\kern #1pt}
\def\zero{\raise1.4pt\hbox{$\scriptscriptstyle\circ$}}
\def\separator{\centerline{---------------------------------}}
\def\dblhbreak{\bigskip\hrule\vskip2pt\hrule\bigskip}

\outer\long\def\ignore#1{}
\def\turnpage{\vfill\eject}

\def\Vee{{\scriptscriptstyle \vee}}
\def\pplus{{\scriptscriptstyle ++}}
\def\plus{{\scriptscriptstyle +}}
\def\minus{{\scriptscriptstyle -}}
\def\mminus{{\scriptscriptstyle --}}
\def\pp#1{{\frenchspacing pp. #1}}
\def\fraction#1#2{\raise1pt\hbox{$#1$}/\raise-1pt\hbox{$#2$}}

\def\boxit#1{\vbox{\hrule\hbox{\vrule\kern2pt
      \vbox{\kern2pt#1\kern2pt}\kern2pt\vrule}\hrule}}

\def\foxit#1#2{\vbox{\null\hbox{\null\kern#2
      \vbox{\kern#2#1\kern#2}\kern#2\null}}}

% --- real output, finally ---------------------------------------------------

\input macros/colordvi
\input macros/epsf
\input macros/amssym.def
% important to input my font defs after the ams ones
\input macros/psfont.defs
% \input macros/font.defs
\input macros/eulerfont.defs

\advance\voffset by \baselineskip
\advance\vsize by -\baselineskip
\nopagenumbers
\raggedbottom

\hsize=6.25truein
\hoffset=0.25truein
\parskip=6pt
\parindent=0pt

\def\endremarks{\smallskip\nobreak\centerline{\raise0.5pt\hbox{$\scriptstyle\circ$}\k{2}-------------\k{2}\raise0.5pt\hbox{$\scriptstyle\circ$}}\medbreak}

% ------------------------------------------------

% \input LABELS
\input \labelsfile
\newwrite\satzlblsout
\immediate\openout\satzlblsout=\labelsfile.tex

\newwrite\tocout
\newwrite\toc

% in proofmode, references are flagged -------------------

\newif\ifproofmode
\proofmodefalse



==> macros/satzen.tex <==

% - theorems ----------------------------

\font\marginbf=cmssbx10 at 8pt

\def\equationitem#1{(%
	\ifinchapter\Romannumeral{\the\chapterno}.\fi%
	\ifinapp \appname.\fi%
	\ifinsec\the\secno.\fi%
	\ifinsubsec\the\subsecno.\fi%
	\the#1)}

\def\alignedequation#1{
\global\advance\satzno by 1
%
\ifinapp
  \immediate\write\satzlblsout{%
  \noexpand\expandafter%
  \noexpand\def%
  \noexpand\csname satz#1\endcsname%
  % {\tokstostring \equationitem{\satzno} }}
  {\equationitem{\satzno}}}
  \immediate\write\satzlblsout{%
  \noexpand\expandafter%
  \noexpand\def%
  \noexpand\csname localsatz#1\endcsname%
  %{\tokstostring \equationitem{\satzno} }}
  {\equationitem{\satzno}}}
  \ifproofmode\margininsert{{\marginbf [#1] }}\fi
% --- text at last -------------------------------------
  \hbox{\bold \equationitem{\satzno} }
%
\else
  \immediate\write\satzlblsout{%
  \noexpand\expandafter%
  \noexpand\def%
  \noexpand\csname satz#1\endcsname%
  % {\tokstostring \equationitem{\satzno} }}
  {\equationitem{\satzno} }}
  \immediate\write\satzlblsout{%
  \noexpand\expandafter%
  \noexpand\def%
  \noexpand\csname localsatz#1\endcsname%
  %{\tokstostring \equationitem{\satzno} }}
  {\equationitem{\satzno}}}
  \ifproofmode\margininsert{{\marginbf [#1] }}\fi
% --- text at last -------------------------------------
  \hbox{\bold \equationitem{\satzno}}
\fi}

% - equation -----------------------------------------

\def\equation#1{
% \immediate\write16{XXXXXXXXXXXXXXXXXXXXXXXXX}
\global\advance\satzno by 1
%
\ifinapp
  \immediate\write\satzlblsout{%
  \noexpand\expandafter%
  \noexpand\def%
  \noexpand\csname satz#1\endcsname%
  % {\tokstostring \equationitem{\satzno} }}
  {\equationitem{\satzno}}}
  \immediate\write\satzlblsout{%
  \noexpand\expandafter%
  \noexpand\def%
  \noexpand\csname localsatz#1\endcsname%
  %{\tokstostring \equationitem{\satzno} }}
  {\equationitem{\satzno}}}
  \ifproofmode\margininsert{{\marginbf [#1] }}\fi
% --- text at last -------------------------------------
  \leqno \hbox{\bold \equationitem{\satzno} }
%
\else
  \immediate\write\satzlblsout{%
  \noexpand\expandafter%
  \noexpand\def%
  \noexpand\csname satz-\filename-#1\endcsname%
  % {\tokstostring \equationitem{\satzno} }}
  {\equationitem{\satzno} }}
  \immediate\write\satzlblsout{%
  \noexpand\expandafter%
  \noexpand\def%
  \noexpand\csname localsatz-\filename-#1\endcsname%
  %{\tokstostring \equationitem{\satzno} }}
  {\equationitem{\satzno}}}
  \ifproofmode\margininsert{{\marginbf [#1] }}\fi
% --- text at last -------------------------------------
  \leqno \hbox{\bold \equationitem{\satzno}}
\fi}

% --- example -------------------------------------------------------

\long\def\example#1{
\satz{#1}{Example}{}}

% --- definition -------------------------------------------------------

\long\def\definition#1#2{
\satz{#1}{Definition}{#2}}

% --------------------------------------------------------------------
% ?name type body
% \outer

\long\def\satz#1#2#3{
\advance\satzno by 1
%
\ifinapp
%
  \immediate\write\satzlblsout{%
  \noexpand\expandafter%
  \noexpand\def%
  \noexpand\csname satz-\filename-#1\endcsname%
  {\tokstostring #2 \appname.\ifinsec\the\secno.\fi%
	\ifinsubsec\the\subsecno.\fi\the\satzno }}%
%
  \immediate\write\satzlblsout{%
  \noexpand\expandafter%
  \noexpand\def%
  \noexpand\csname localsatz-\filename-#1\endcsname%
  {\tokstostring #2 \appname.\ifinsec\the\secno.\fi%
	\ifinsubsec\the\subsecno.\fi\the\satzno }}
  \ifproofmode\margininsert{{\marginbf [#1] }}\fi
% --- text at last -------------------------------------
  {\bold #2 \appname.\ifinsec\the\secno.\fi%
	\ifinsubsec\the\subsecno.\fi\the\satzno.}\ {\sl #3 }
%
\else
%
  \immediate\write\satzlblsout{%
  \noexpand\expandafter%
  \noexpand\def%
  \noexpand\csname satz-\filename-#1\endcsname%
  {\tokstostring #2 \ifinchapter\Romannumeral{\the\chapterno}.\fi\ifinsec\the\secno.\fi%
	\ifinsubsec\the\subsecno.\fi\the\satzno }}%
%
  \immediate\write\satzlblsout{%
  \noexpand\expandafter%
  \noexpand\def%
  \noexpand\csname localsatz-\filename-#1\endcsname%
  {\tokstostring #2 \ifinchapter\Romannumeral{\the\chapterno}.\fi\ifinsec\the\secno.\fi%
	\ifinsubsec\the\subsecno.\fi\the\satzno }}
  \ifproofmode\margininsert{{\marginbf [#1] }}\fi
% --- text at last -------------------------------------
  {\bold \ifinchapter\Romannumeral{\the\chapterno}.\fi\ifinsec\the\secno.\fi%
\ifinsubsec\the\subsecno.\fi\the\satzno.\kern4pt #2.}\ {\sl #3 }%
\fi}

\outer\long\def\theorem#1#2{\satz{#1}{Theorem}{#2}}
\outer\long\def\lemma#1#2{\satz{#1}{Lemma}{#2}}
\outer\long\def\proposition#1#2{\satz{#1}{Proposition}{#2}}
\outer\long\def\corollary#1#2{\satz{#1}{Corollary}{#2}}

% --- for imported files ----------------------------------------------

% #1 = external file
\def\reftosatz#1#2{%
\immediate\write16{*** satz-#1-#2 ***}%
\ifproofmode%
\expandafter%
\ifx\csname satz-#1-#2\endcsname\relax%
\margininsert{$\spadesuit$ {\marginbf [#2]\ }}\rlap{$\bullet$}%
\else \margininsert{\BrickRed{$\heartsuit$} {\marginbf [#2]\ }}\fi%
\fi\csname satz-#1-#2\endcsname}

% --- for internal reference --------------------------------------------

\def\lreftosatz#1{%
\reftosatz{\filename}{#1}}
% \ifproofmode
% \expandafter%
% \ifx\csname localsatz-\filename-#1\endcsname\relax%
% \margininsert{$\spadesuit$ {\marginbf [#1]\ }}\rlap{$\bullet$}%
% \else\margininsert{\BrickRed{$\heartsuit$} {\marginbf [#1]\ }}\fi%
% \fi
% \csname localsatz-\filename-#1\endcsname}


